Enhancing disease detection in radiology reports through fine-tuning lightweight LLM on weak labels

Despite significant progress in applying large language models (LLMs) to the medical domain, several limitations still prevent them from practical applications. Among these are the constraints on model size and the lack of cohort-specific labeled datasets. In this work, we investigated the potential of improving a lightweight LLM, such as Llama 3.1-8B, through fine-tuning with datasets using synthetic labels. Two tasks are jointly trained by combining their respective instruction datasets. When the quality of the task-specific synthetic labels is relatively high (e.g., generated by GPT4- o), Llama 3.1-8B achieves satisfactory performance on the open-ended disease detection task, with a micro F1 score of 0.91. Conversely, when the quality of the task-relevant synthetic labels is relatively low (e.g., from the MIMIC-CXR dataset), fine-tuned Llama 3.1-8B is able to surpass its noisy teacher labels (micro F1 score of 0.67 v.s. 0.63) when calibrated against curated labels, indicating the strong inherent underlying capability of the model. These findings demonstrate the potential of fine-tuning LLMs with synthetic labels, offering a promising direction for future research on LLM specialization in the medical domain.

==> tables/tab_classification1.tex <==
\begin{table}
    \caption{Performance of micro-precision, micro-recall, and micro-F1 scores in the multiple-choice disease classification task on MIMIC data.}
    \label{joint_mimic}
    \centering
    \begin{tabular}{lrrrrrrrr} \toprule
 & \multicolumn{2}{c}{Training sample} &\multicolumn{3}{c}{Human-curated label}& \multicolumn{3}{c}{NegBio-generated label} \\ \cmidrule(rl){2-3}\cmidrule(rl){4-6}\cmidrule(rl){7-9}
 Model & NIH/MIRDC & MIMIC & Accuracy& Recall& F1&Accuracy& Recall& F1\\ \midrule
Llama 3.1 Instruct-8B\\
\hspace{1em} 0 (Baseline) & 0 & 0 &0.46&0.65&0.54&0.33&0.75&0.46\\ 
\hspace{1em} 1,500 & 1,000 & 500&0.44&0.62&0.51&0.30&0.67&0.41\\
\hspace{1em} 3,000 & 2,000 & 1,000&0.45&0.64&0.53&0.30&0.69&0.42\\ 
\hspace{1em} 4,500 & 3,000 & 1,500&0.53&0.67&0.59&0.35&0.71&0.47\\ 
% 2e-3, 4e-5 not working
\hspace{1em} 7,500 & 5,000 & 2,500&0.61&0.72&0.66&0.41&0.77&0.54\\ 
\hspace{1em} 9,000 & 6,000 & 3,000& 0.62& 0.72&0.67&0.44&0.83&0.58\\
\hspace{1em} 13,500 & 9,000 & 4,500& 0.69&0.59&0.64&0.55&0.74&0.63\\ 
NegBio &-&-&0.82&0.51&0.63&-&-&-\\ 
GPT4-o&-&-&0.83&0.89&0.86&0.50&0.85&0.63\\ \bottomrule
    \end{tabular}
\end{table}

==> tables/tab_lr1.tex <==
\begin{table}
    \caption{Performance of Llama 3 Instruct-8B on the multiple-choice disease classification task using micro-accuracy, micro-recall, and micro-F1 scores. The model was trained on 100,000 samples from the MIMIC-CXR dataset and then tested on human-curated data from the same MIMIC-CXR source.}
    \label{mimic_yishu}
    \centering
    \begin{tabular}{rrrrrrr} \toprule
 \multirow{2}{*}{\makecell[r]{Learning \\ rate}} & \multicolumn{3}{c}{NegBio label}& \multicolumn{3}{c}{Curated label}     \\ \cmidrule(rl){2-4}\cmidrule(rl){5-7}
 & Accuracy& Recall& F1&Accuracy& Recall& F1\\ \midrule
0.00 &0.33&0.75&0.46&0.46&0.65&0.54\\ 
7e-6&0.39&0.75&0.51&0.56&0.67&0.61\\
9e-6&0.38&0.78&0.51&0.55&0.70&0.62\\ 
1e-5&0.44&0.8&0.57&0.64&\textbf{0.72}&\textbf{0.68}\\ 
% 2e-3, 4e-5 not working
8e-5&0.71&0.8&0.75&0.81&0.56&0.66\\ 
3e-4&0.89&0.92&0.90&0.84&0.54&0.66\\ 
% MIMIC label&NA&1.00&1.00&1.00&0.82&\textbf{0.51}&\textbf{0.63}\\ 
% GPT4-o&NA&0.50&0.85&0.63&0.83&0.89&0.86\\ 
\bottomrule
    \end{tabular}
\end{table}

==> tables/tab_lr2.tex <==
\begin{table}
\caption{Performance of \sllm on the multiple-choice disease classification task using micro-precision, micro-recall, and micro-F1 scores. The model was trained on 100,000 samples from the MIMIC-CXR dataset and then tested on human-curated data from the same MIMIC-CXR source.}
\label{tab:mimic_yishu_lr}
\centering
\vspace{-1em}
\begin{tabular}{rrrr} 
\toprule
Learning rate & Precision & Recall& F1\\ 
\midrule
0.00 &0.46&0.65&0.54\\ 
7e-6&0.56&0.67&0.61\\
9e-6&0.55&0.70&0.62\\ 
1e-5&0.64&0.72&0.68\\ 
% 2e-3, 4e-5 not working
8e-5&0.81&0.56&0.66\\ 
3e-4&0.84&0.54&0.66\\ 
% MIMIC label&NA&1.00&1.00&1.00&0.82&\textbf{0.51}&\textbf{0.63}\\ 
% GPT4-o&NA&0.50&0.85&0.63&0.83&0.89&0.86\\ 
\bottomrule
    \end{tabular}
\end{table}
